Probing Factual Knowledge Transfer with Training Data Interventions

Do multilingual language models transfer factual knowledge across languages during continued pretraining, or do they mostly recall facts learned directly from the target-language data? To answer this question more reliably, we propose an intervention-based framework: starting from an English-pretrained model, we continue pretraining on Persian data from which specific facts have been systematically removed at varying levels of granularity. We construct SIFT, a resource of 500 triples across 20 relations, stratified by the cultural origin of each fact's subject into general (globally prominent) and Persian-related entities, designed for both systematic fact removal from training data and evaluation, with natively written Persian cloze templates. Our results show that fact transfer is very limited: under the strictest removal condition, a large majority of English-acquired facts fail to transfer into Persian. We further show that sentence-level co-occurrence removal is insufficient to eliminate fact signal, and that easier (randomly selected) negative candidate sets substantially inflate apparent transfer by rewarding shallow associative heuristics, while performance on a harder candidate set that allows for less reliance on heuristics is much lower. Finally, we show that source-language entity frequency has a large influence, with Persian-related facts, which are orders of magnitude rarer in the English corpus, hardly transferring.

==> causal_graph.tex <==
% Requires: \usepackage{tikz}
% Optional: \usetikzlibrary{positioning, arrows.meta, calc}

\begin{figure}[t]
\centering
\begin{tikzpicture}[
    node distance=2.2cm and 2.4cm,
    box/.style={
        rectangle, rounded corners=4pt, draw, thick,
        minimum width=3.2cm, minimum height=1.1cm,
        align=center, font=\small
    },
    data/.style={box, fill=blue!8, draw=blue!40},
    blocked/.style={box, fill=teal!8, draw=teal!40},
    heuristic/.style={box, fill=orange!8, draw=orange!40},
    outcome/.style={box, fill=gray!10, draw=gray!50},
    open arrow/.style={-{Stealth[length=5pt]}, thick, blue!60},
    blocked arrow/.style={-{Stealth[length=5pt]}, thick, dashed, gray!60},
    feed arrow/.style={-{Stealth[length=5pt]}, thin, black!50},
    xmark/.style={red!70!black, line width=1.8pt},
]

% Top row: pretraining datasets
\node[data] (en-data) {EN pretraining\\data};
\node[blocked, right=2.8cm of en-data] (fa-data) {FA pretraining\\data};

% Middle row: causal mediators
\node[data, below left=2cm and 0.8cm of en-data] (en-facts) {Facts in EN\\\scriptsize\textit{present}};
\node[blocked, below right=2cm and -0.6cm of en-data] (fa-facts) {Facts in FA\\\scriptsize\textit{removed}};
\node[heuristic, below right=2cm and 0.8cm of fa-data] (heuristics) {Shallow heuristics\\\scriptsize\textit{from both corpora}};

% Bottom: outcome
\node[outcome, below=2.5cm of fa-facts] (accuracy) {FA factual accuracy\\\scriptsize\textit{observed}};

% Edges: data -> mediators
\draw[feed arrow] (en-data) -- (en-facts);
\draw[feed arrow] (fa-data) -- (fa-facts);
\draw[feed arrow, dashed] (en-data) -- (heuristics);
\draw[feed arrow, dashed] (fa-data) -- (heuristics);

% Edge: EN facts -> accuracy (open path)
\draw[open arrow] (en-facts) -- node[midway, left, font=\small\itshape, text=blue!60] {transfer?} (accuracy);

% Edge: FA facts -> accuracy (blocked)
\draw[blocked arrow] (fa-facts) -- (accuracy);

% Edge: heuristics -> accuracy (blocked)
\draw[blocked arrow] (heuristics) -- (accuracy);

% X marks on blocked paths
% FA facts path
\coordinate (mid-fa) at ($(fa-facts.south)!0.5!(accuracy.north)$);
\draw[xmark] ($(mid-fa)+(-0.18,0.18)$) -- ($(mid-fa)+(0.18,-0.18)$);
\draw[xmark] ($(mid-fa)+(0.18,0.18)$) -- ($(mid-fa)+(-0.18,-0.18)$);
\node[right=0.3cm of mid-fa, font=\scriptsize, text=red!70!black, align=left] {blocked by\\removal};

% Heuristics path
\coordinate (mid-h) at ($(heuristics.south)!0.5!(accuracy.north east)$);
\draw[xmark] ($(mid-h)+(-0.18,0.18)$) -- ($(mid-h)+(0.18,-0.18)$);
\draw[xmark] ($(mid-h)+(0.18,0.18)$) -- ($(mid-h)+(-0.18,-0.18)$);
\node[right=0.3cm of mid-h, font=\scriptsize, text=red!70!black, align=left] {controlled by\\hard candidates};

\end{tikzpicture}
\caption{Causal graph of our experimental design. Three paths could explain Persian factual accuracy: cross-lingual transfer from English knowledge (solid), direct memorization from Persian data (dashed), and shallow heuristics from both corpora (dashed). Our training data intervention blocks the memorization path, and hard candidate evaluation controls for heuristic shortcuts, isolating cross-lingual transfer as the only remaining explanation for correct Persian recall.}
\label{fig:causal-graph}
\end{figure}


==> causal_graph_with_example.tex <==
% Uses the same style as Figure 1.
% Requires: \usepackage{tikz}
% \usetikzlibrary{positioning, arrows.meta, calc}
% Compile with XeLaTeX

\begin{figure}[t]
\centering
\definecolor{yellowfill}{HTML}{EBCB8B}
\definecolor{greenfill}{HTML}{A3BE8C}
\definecolor{bluefill}{HTML}{5E81AC}
\definecolor{redfill}{HTML}{BF616A}

\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[%
    yscale=1, xscale=0.6,
    block/.style={rectangle, rounded corners, thick, draw=black, align=center, inner sep=6pt},
    en/.style={fill=greenfill!50},
    fa/.style={fill=yellowfill!50},
    probe/.style={fill=redfill!30},
    modelbox/.style={fill=bluefill!50},
    X/.tip={Triangle[]},
    arrow/.style={thick, rounded corners},
    annot/.style={fill=white, font=\sffamily\normalsize, anchor=center},
    xmark/.style={redfill, line width=2pt},
]

% Top row: corpora — pushed to edges
\node[block, en, minimum width=4cm, minimum height=1cm, font=\sffamily\bfseries\large] 
    (en-corpus) at (-0.2, 0) {English Corpus};
\node[block, fa, minimum width=4cm, minimum height=1cm, font=\sffamily\bfseries\large] 
    (fa-corpus) at (8.2, 0) {Persian Corpus};

% Middle row: facts — pushed to edges
\node[block, en, minimum width=4.6cm, minimum height=2.2cm] 
    (en-facts) at (-0.2, -2.8) {%
    {\sffamily\bfseries\normalsize Facts in EN} — {\small\itshape present}\\[4pt]
    {\normalsize Einstein died in \textbf{Princeton}.}%
};

\node[block, fa, minimum width=4.6cm, minimum height=2.2cm] 
    (fa-facts) at (8.2, -2.8) {%
    {\sffamily\bfseries\normalsize Facts in FA} — {\small\itshape removed}\\[4pt]
    {\normalsize\foreignlanguage{arabic}{اینشتین در \textbf{پرینستون} درگذشت.}}%
};

% Outcome: centered
\node[block, modelbox, minimum width=5cm, minimum height=1cm] 
    (acc) at (4, -5.8) {%
    {\sffamily\bfseries\normalsize Persian Fact Recall} — {\small\itshape observed}%
};

% Bottom: shallow cues — full width
\node[block, probe, minimum width=7cm, minimum height=2.2cm] 
    (heur) at (4, -8.6) {%
    {\sffamily\bfseries\normalsize Shallow Cues}\\[4pt]
    {\normalsize Hard: Ulm, Zurich, Bern, Berlin, Washington}\\[2pt]
    {\normalsize\foreignlanguage{arabic}{اولم، زوریخ، برن، برلین، واشنگتن}}%
};

% Corpus -> Facts
\draw[-X, arrow] (en-corpus) -- (en-facts);
\draw[-X, arrow] (fa-corpus) -- (fa-facts);

% Facts -> Accuracy
\draw[-X, arrow, draw=greenfill!80!black] (en-facts) -- (acc)
    node[pos=0.5, annot, text=greenfill!80!black] {transfer};
\draw[-X, arrow, dashed, draw=black!40] (fa-facts) -- (acc)
    node[pos=0.5, annot, text=black!50] {direct};

% X on FA facts path
\coordinate (mf) at ($(fa-facts.south)!0.5!(acc.north)$);
\draw[xmark] ($(mf)+(-0.18,0.18)$) -- ($(mf)+(0.18,-0.18)$);
\draw[xmark] ($(mf)+(0.18,0.18)$) -- ($(mf)+(-0.18,-0.18)$);

% Shallow cues -> Accuracy
\draw[-X, arrow, dashed, draw=black!40] (heur) -- (acc);

% X on heuristics path
\coordinate (mh) at ($(heur.north)!0.5!(acc.south)$);
\draw[xmark] ($(mh)+(-0.18,0.18)$) -- ($(mh)+(0.18,-0.18)$);
\draw[xmark] ($(mh)+(0.18,0.18)$) -- ($(mh)+(-0.18,-0.18)$);

% Curved arrows from corpora to shallow cues
\draw[-X, arrow, dashed, draw=black!30] (en-corpus.west) to[out=220, in=160] (heur.west);
\draw[-X, arrow, dashed, draw=black!30] (fa-corpus.east) to[out=-40, in=20] (heur.east);

\end{tikzpicture}%
}
\caption{Causal graph of our experimental design. Three paths could explain Persian factual recall: cross-lingual transfer from English (solid), direct memorization from Persian data (dashed), and shallow cues from both corpora (dashed, curved). Removal blocks memorization; hard candidates control shallow cues, isolating transfer.}
\label{fig:causal-graph}
\end{figure}

==> fig_schematic.tex <==
% \begin{figure}
%     \centering
%     \definecolor{yellowfill}{HTML}{EBCB8B}
%     \definecolor{greenfill}{HTML}{A3BE8C}
%     \definecolor{bluefill}{HTML}{5E81AC}

%     \begin{tikzpicture}[%
%         yscale=1,xscale=1,every node/.style={scale=0.8},
%         node distance=1.2cm,
%         %
%         block/.style={rectangle, rounded corners, thick, draw=black, align=center, inner sep=6pt},
%         example/.style={block, minimum width=6cm},
%         en/.style={fill=greenfill!50},
%         fa/.style={fill=yellowfill!50},
%         exlabel/.style={anchor=south west, font=\sffamily\bfseries},
%         %
%         model/.style={block, fill=bluefill!50, font=\bfseries},
%         %
%         X/.tip={Triangle[]},
%         arrow/.style={thick,rounded corners},
%         annot/.style={fill=white, font=\sffamily\bfseries, scale=.9, anchor=center},
%         ]

%         \node[example,en] (en)  at (0,  0)  {\textbf{Albert Einstein} was a \textbf{physicist}.};
%         \node[shift=(en.north west), exlabel] {EN data};

%         \node[example,fa]  (fa) at (0, -2.5) {\foreignlanguage{arabic}{\sout{\textbf{آلبرت اینشتین} یک \textbf{فیزیک‌دان} بود.}}};
%         \node[shift=(fa.north west), exlabel] {FA data};

%         \node[] (triple) at (0, -.6) {$\langle$Albert Einstein, field of work, physics$\rangle$};
%         \draw[-X,arrow] (triple) -- (fa) node[pos=0.35,annot] {fact removal};

%         \node[model] (enmodel) at (4, 0) {EN};
%         \node[shift=(enmodel.north), exlabel, anchor=south] {Model};
%         \node[model] (famodel) at (4, -2.5) {FA};

%         \draw[-X,arrow] (en) -- (enmodel) node[pos=0.45,annot] {\faCogs};
%         \draw[-X,arrow] (fa) -- ($(fa.east)+(.5,0)$) -- ++(0, 1.6) -- (famodel.north |- {$(fa.east)+(0,1.6)$} -| famodel) -- (famodel.north);
%         \draw[-,arrow] (enmodel) -- (famodel) node[pos=0.66,annot] {\faCogs};
%     \end{tikzpicture}
%     \caption{Schematic illustration of our intervention-based approach.  We identify facts in the English pre-training data, then systematically remove them from the Farsi pre-training data before continued pre-training.  Finally, we probe the resulting model for knowledge of the removed fact. \textcolor{red}{maybe the probing/scoring could also be illustrated below the ``FA'' model?}}
%     \label{fig:schematic}
% \end{figure}

\begin{figure}
    \centering
    \definecolor{yellowfill}{HTML}{EBCB8B}
    \definecolor{greenfill}{HTML}{A3BE8C}
    \definecolor{bluefill}{HTML}{5E81AC}
    \definecolor{redfill}{HTML}{BF616A}
    
    \begin{tikzpicture}[%
        yscale=1,xscale=1,every node/.style={scale=0.8},
        %
        block/.style={rectangle, rounded corners, thick, draw=black, align=center, inner sep=6pt},
        example/.style={block, minimum width=5.2cm},
        en/.style={fill=greenfill!50},
        fa/.style={fill=yellowfill!50},
        probe/.style={fill=redfill!30},
        exlabel/.style={font=\sffamily\bfseries},
        %
        model/.style={block, fill=bluefill!50, font=\bfseries, minimum width=1.6cm, minimum height=0.7cm},
        %
        X/.tip={Triangle[]},
        arrow/.style={thick,rounded corners},
        annot/.style={fill=white, font=\sffamily\small, anchor=center},
        ]
    
        %% ── Stage 1: English pretraining ──
        \node[example,en] (en) at (0, 0) {%
            \textbf{Einstein} was a \textbf{physicist}.\\[2pt]
            \textbf{Einstein} won the Nobel Prize.
        };
        \node[exlabel, above=0.1cm of en] {English pretraining data};
    
        \node[model] (base) at (4.8, 0) {ٍEN-Base LM};
        \draw[-X,arrow] (en) -- (base) node[pos=0.5,annot] {pretrain};
    
        %% ── Stage 2: Persian CPT ──
        \node[example,fa] (fa) at (0, -2.8) {%
            \foreignlanguage{arabic}{%
                \sout{\textbf{اینشتین} یک \textbf{فیزیک‌دان} بود.}%
            }%
            \hspace{0.1cm}{\scriptsize\itshape\textcolor{redfill}{removed}}\\[4pt]
            \foreignlanguage{arabic}{%
                \textbf{اینشتین} جایزه نوبل برد.%
            }%
            \hspace{0.1cm}{\scriptsize\itshape\textcolor{black!50}{kept}}
        };
        \node[exlabel, above=0.1cm of fa] {Persian CPT data};
    
        \node[model] (cpt) at (4.8, -2.8) {CPT LM};
        \draw[-X,arrow] (fa) -- (cpt) node[pos=0.5,annot] {CPT};
        \draw[-X,arrow] (base) -- (cpt) node[pos=0.5,annot,anchor=west,xshift=2pt] {init};
    
        %% ── Triple + filter arrow BELOW the FA box ──
        \node[block, draw=redfill, fill=redfill!15, font=\small] (triple) 
            at (0, -5) {%
            $\langle$Einstein, field\_of\_work, physics$\rangle$%
        };
        \draw[-X, thick, draw=redfill, dashed] 
            (triple.north) -- (fa.south)
            node[pos=0.5, right, font=\small\sffamily, text=redfill!80!black, xshift=2pt] 
            {filter};
    
        %% ── Stage 3: Probing ──
        \node[example, probe, minimum width=5.2cm] (probeq) at (0, -6.8) {%
            \foreignlanguage{arabic}{%
                حوزه کاری اینشتین \rule{1.2cm}{0.4pt} است.%
            }\\[2pt]
            {\small\itshape Candidates: physics, chemistry, \ldots}%
        };
        \node[exlabel, above=0.1cm of probeq] {Factual probe (Persian)};
    
        \draw[-X,arrow] (probeq.east) -| (cpt.south)
            node[pos=0.25, annot] {evaluate};
    
        %% ── Key question ──
        \node[anchor=west, font=\small\itshape, text=bluefill!80!black, 
              text width=1.8cm, align=left] 
            at ($(cpt.east)+(0.1,0)$) {%
            Did English knowledge\\transfer to Persian?%
        };
    
    \end{tikzpicture}
    
    \caption{Schematic of our experimental setup. A base language model pretrained on English (\textit{top}) is adapted via continued pretraining (CPT) on Persian data from which specific facts have been systematically filtered (\textit{middle}). The resulting model is then probed on the removed facts using Persian cloze templates (\textit{bottom}). Correct recall of a fact absent from the Persian training data but present in the English data constitutes evidence of cross-lingual knowledge transfer.}
    \label{fig:schematic}
\end{figure}

==> removed.tex <==
% Specifically, we investigate the following research questions:
% \begin{description}

%     % \item[RQ1] Does factual knowledge transfer from English to Persian through continued pretraining when the relevant facts have been removed from the Persian training data?
    
%     \item[RQ1] What level of target-language data intervention is required to ensure a fact is unseen in the target language, forcing the model to rely on cross-lingual knowledge transfer to answer correctly?
    
%      % \item[RQ2] Are correct predictions after fact removal due to genuine knowledge transfer from English, or does the model rely on surface-level cues such as associating a subject's cultural background with related candidates?

%       \item[RQ2] To what extent do we observe cross-lingual transfer during continued pre-training of an English model on Persian, and how much of it is based on shallow heuristics, as opposed to genuine knowledge transfer?

       

%     % \item[RQ3] Does cross-lingual factual transfer depend on the cultural provenance of the fact, specifically, do facts about globally prominent entities transfer more readily than facts rooted in a source or target cultural context?
    
%     \item[RQ3] How does the cultural origin of a fact affect whether it transfers across languages? For example, do facts about globally well-known entities transfer more easily than facts tied to the target language?
        
% \end{description}

